Situationally Aware Options

Hierarchical abstractions, also known as options -- a type of temporally extended action (Sutton et. al. 1999) that enables a reinforcement learning agent to plan at a higher level, abstracting away from the lower-level details. In this work, we learn reusable options whose parameters can vary, encouraging different behaviors, based on the current situation. In principle, these behaviors can include vigor, defence or even risk-averseness. These are some examples of what we refer to in the broader context as Situational Awareness (SA). We incorporate SA, in the form of vigor, into hierarchical RL by defining and learning situationally aware options in a Probabilistic Goal Semi-Markov Decision Process (PG-SMDP). This is achieved using our Situationally Aware oPtions (SAP) policy gradient algorithm which comes with a theoretical convergence guarantee. We learn reusable options in different scenarios in a RoboCup soccer domain (i.e., winning/losing). These options learn to execute with different levels of vigor resulting in human-like behaviours such as `time-wasting' in the winning scenario. We show the potential of the agent to exit bad local optima using reusable options in RoboCup. Finally, using SAP, the agent mitigates feature-based model misspecification in a Bottomless Pit of Death domain.

==> algorithm.tex <==
%Algorithm


\vspace{-0.2cm}
\section{Preliminaries}
\vspace{-0.3cm}
%A robust MDP is defined as the $5$-tuple $M_{R}=\langle X,A,R,\gamma, \mathcal{P}\rangle$ where $X$ is a set of finite states, $A$ is a set of actions, $\mathcal{P}$
%denotes a known uncertainty set over state-action-next-state transitions and $R:X\times A\rightarrow\mathbb{R}$ is a deterministic and bounded reward function. 

Throughout this paper we make the following assumptions which are standard in Policy Gradient (PG) literature \cite{Bhatnagar2009}: \textit{Assumption (A1)} Under any policy $\pi$, the Markov chain resulting from the Robust MDP is irreducible and aperiodic. \textit{Assumption (A2)} A policy $\pi_\theta(x,a)$ for any $x\in X$, $a \in A$ pair is continuously differentiable with respect to the parameter $\theta$. \textit{Assumption (A3)} The optimal value function $V^*$ is found within the hypothesis space of function approximators that are being utilized. We use these standard assumptions to define the robust transition probability function and the robust steady-state distribution for the discounted setting. We then use these definitions to derive the robust policy gradient version of Equation \ref{eqn:policy_gradient}. 

%\subsubsection{Robust Transition Probability Distribution: }

\textbf{\underline{Robust Transition Probability Distribution:}} The robust value function is defined for a policy $\pi:X\rightarrow A$ as ${V^{\pi}(x)=r(x,\pi(x))+\gamma\inf_{p\in\mathcal{P}}\mathbb{E}^{p}[V^{\pi}(x')\vert x,\pi ]}$ and the robust action value function is given by ${Q^{\pi}(x,a)=r(x,a)+\gamma\inf_{p\in\mathcal{P}}\mathbb{E}^{p}[V^{\pi}(x')\vert x,a,\pi]}$ where ${\hat{p}_{min}(x' \vert x,a)=\arg\inf_{p\in\mathcal{P}}\mathbb{E}^{p}[V^{\pi}(x')\vert x,a,\pi]}$. Here, $\hat{p}_{min}(x' \vert x,a)$ is the transition probability distribution that minimizes the expected return $\mathbb{E}^{p}[V^{\pi}(x')\vert x,a,\pi]$ for a given state $x$ and action $a$ and belongs to the pre-defined uncertainty set $\mathcal{P}$. Since $\hat{p}_{min}(x' \vert x,a)$ is selected independently for each state  we can construct a stochastic matrix $\hat{P}_{min}$ where each row is defined by $\pi^{\top}\hat{p}_{min}(x' \vert x,\cdot)$.


%\subsubsection{Robust Steady-State Distribution: }
\textbf{\underline{Robust State Distribution: }} The matrix $\hat{P}_{min}$ can be interpreted as an adversarial distribution in a zero-sum game if the adversary fixes its worst case strategy \cite{Filar2012}. 

%It has also been shown  previously for zero-sum games that the optimal strategy of an adversary is stationary \cite{Filar2012,Iyenger2005}. As a result, in the limit, the robust state distribution, defined in Equation \ref{eq:statedistribution}, is stationary.

\begin{define}

Given the initial state distribution $\mu$, the robust discounted
state distribution is: ${\hat{d}^{\pi}(x)= \int\mu(x_{0})\sum_{t=0}^{\infty}\gamma^{t}\hat{P}_{min}^t(x|x_{0})dx_{0}}$.
\end{define}
%\begin{equation}
%\hat{d}^{\pi}(x)=\int\mu(x_{0})\sum_{t=0}^{\infty}\gamma^{t}\hat{P}_{min}^{t}(x|x_{0})dx_{0}.\label{eq:statedistribution}
%\end{equation}
%\end{define}

The robust discounted state distribution is the same as the  state distribution used by \cite{Sutton2000} for the discounted setting. However, the transition kernel is selected robustly rather than assumed to be the transition kernel of the target MDP. The robust discounted state distribution $\hat{d}^{\pi}(x)$ intuitively represents executing the transition probability model that leads the agent to the worst (i.e., lowest value) areas of the state space. 

\vspace{-0.1cm}
\section{Robust Policy Gradient}
\label{sec:rac-pg}
\vspace{-0.1cm}
Using the above definitions, we can now derive the Robust Policy Gradient (R-PG) for the discounted setting, which is used for policy improvement in ROPI. \footnote{Similar results are obtained for the average reward setting.}. To derive the R-PG, we (1) define the robust performance objective; (2) Derive the corresponding robust compatibility conditions which enables us to incorporate a function approximator into the policy gradient.


%learns a robust policy to model uncertainty whilst maximizing a robust objective function. In order to develop this robust algorithm, we need to (1) define the robust performance objective; (2) derive a robust gradient with respect to this objective; (3) derive the corresponding compatibility conditions to ensure that this algorithm can be used with function approximation; (4) Show that the gradient is unbiased. 

%It then follows that this algorithm converges using a two-time scale stochastic approximation algorithm as developed by \cite{Bhatnagar2009}. Note that full proofs can be found in the supplementary material unless otherwise stated.


%\subsection{Robust Performance Objective}
%\label{sec:robustobjective}
\textbf{\underline{Robust Performance Objective:}} R-PG optimizes the discounted expected reward objective ${J(\pi)=\inf_p \mathbb{E}^p [\sum_{t=1}^\infty \gamma^{t-1}r_t \vert x_0, \pi, \mathcal{P} ]}$ where $\mathcal{P}$ is a given uncertainty set; $\gamma \in [0,1]$ is a discount factor and $r_t$ is a bounded reward at time $t$. Next we define the robust value function as ${\tilde{Q}^{\pi}(x,a)=\inf_{p\in\mathcal{P}}\mathbb{E}^{p}[\sum_{t=0}^{\infty}\gamma^{t} r_{t+1}\vert x_{0}=x,a_{0}=a,\pi]}$ and we denote the robust expected reward as $
{\tilde{V}^{\pi}(x)=\sum_{a\in A}\pi(x,a)Q^{\pi}(x,a)}$. The robust policy $\pi_{\theta}:X\rightarrow \Delta_A$ is parameterized
by the parameters $\theta\in\mathbb{R}^{d}$. We wish to maximize
$J(\pi_{\theta})$ to obtain the optimal set of policy parameters $\theta^{*}=\arg\max_{\theta}J(\pi_{\theta})$

%\subsection{Robust Policy Gradient}
%\label{sec:gradient}
\textbf{\underline{Robust Policy Gradient:}} Given the robust performance objective with respect to the robust discounted state distribution, we can now derive the robust policy gradient with respect to the robust policy $\pi_{\theta}$. $\pi$ is parameterized by $\theta$ unless otherwise stated. As in \cite{Sutton2000}, we derive the gradient using the robust formulation for the discounted scenario. The discounted expected reward case is presented as Lemma \ref{lemma:lemmagradavg}. The main differences between this Lemma and that of \cite{Sutton2000} is that we incorporate the robust state distribution $\hat{d}^{\pi}$ and emit a transition distribution $\hat{p}_{min}$ leading the agent to the areas of lowest value at each timestep.


\begin{lemma}
\label{lemma:lemmagradavg}
Suppose the we are maximizing the robust performance objective ${J(\pi)=\inf_{p\in\mathcal{P}}\mathbb{E}^{p}[\sum_{t=0}^{\infty}\gamma^{t-1}r_{t}\vert x_{0},\pi]}$
from a given start state $x_{0}\in X$ with respect to a policy ${\pi_{\theta}:X\rightarrow\Delta_{A}}$
parameterized by $\theta\in\mathbb{R}^{d}$ and the robust action
value function is defined as ${Q^{\pi}(x,a)=\inf_{p\in\mathcal{P}}\mathbb{E}^{p}[\sum_{t=0}^{\infty}\gamma^{t-1}r_{t}\vert x_{t}=x,a_{t}=a,\pi]}$.
Then the gradient with respect to the performance objective is:

\vspace{-0.3cm}
\begin{equation}
\frac{\partial J(\pi)}{\partial\theta}=\sum_{x}\hat{d}^{\pi}(x)\sum_{a}\frac{\partial\pi(x,a)}{\partial\theta}\tilde{Q}^{\pi}(x,a) \enspace .
\end{equation}
%where $\hat{d}^{\pi}(x)=\sum_{t=0}^{\infty}\gamma^{t}\hat{p}(x\rightarrow y,k,\pi)$
%is the state distribution for $\hat{p}(x\rightarrow y,k,\pi)$,
%which represents the probability that the agent will transition from
%state $x$ to $y$ after $k$ timesteps under policy $\pi$.
\end{lemma}

The vectorized robust gradient update is therefore 
$\nabla_{\theta}J(\pi_{\theta})=\sum_{y}\hat{d}^{\pi}(x)\sum_{a}\nabla_{\theta}\pi_{\theta}(x,a)\tilde{Q}^{\pi}(x,a)$. It is trivial to incorporate a baseline into the lemma that does not bias the gradient leading to the gradient update equation: $\nabla_{\theta}J(\pi_{\theta})=\sum_{x}\hat{d}^{\pi}(x)\sum_{a}\nabla_{\theta}\pi_{\theta}(x,a)[\tilde{Q}^{\pi}(x,a)\pm b(x)]$.


%\subsection{Robust Compatibility Conditions}
%\label{sec:compatibiity}
\textbf{\underline{Robust Compatibility Conditions:}} The above robust gradient updates do not as yet possess the ability to incorporate function approximation. However, by deriving robust compatibility conditions, we can replace $Q^{\pi}(x,a)$ with a linear function approximator $f_w(x,a)=w^T \psi_{x,a}$. Here $w\in \mathbb{R}^d$ represents the approximator's parameters and $\psi_{x,a}=\nabla\log \pi(x,a)$ which represent the compatible features condition. The robust compatibility features are presented as Lemma \ref{lemma:lemmacompat}. Note that this compatibility condition is with respect to the robust state distribution $\hat{d}^{\pi}$.

\begin{lemma}
\label{lemma:lemmacompat}
Let $f_{w}:X\times A\rightarrow\mathbb{R}$ be an approximation to
$Q^{\pi}(x,a).$ If $f_{w}$ minimizes the mean squared error $e^{\pi}(w)=\sum_{x}\hat{d}^{\pi}(x)\sum_{a\in A}\pi(x,a)[\tilde{Q}^{\pi}(x,a)-f_{w}(x,a)]^{2}$
and is compatible such that it satisifes
$\frac{\partial f_{w}(x,a)}{\partial w}=\frac{\partial\pi(x,a)}{\partial\theta}\frac{1}{\pi(x,a)}$, then
\begin{equation}
\frac{\partial J(\theta)}{\partial\theta}=\sum_{x}\hat{d}^{\pi}(x)\sum_{a}\frac{\partial\pi(x,a)}{\partial\theta}f_{w}(x,a) \enspace .
\end{equation}
\vspace{-0.6cm}

\end{lemma}



%
%\vspace{-0.4cm}
%
%\section{Convergence of Robust AC-PG}
%\label{sec:convergence}
%Given the robust AC-PG setting, we have the following update equations (1) $\hat{J}_{t+1}  =  (1-\epsilon_{t})\hat{J}_{t}+\epsilon_{t}r_{t+1}$, (2) $\delta_{t}  =  r_{t+1}-\hat{J}_{t+1}+v_{t}^{T}f_{x_{t+1}}-v_{t}^{T}f_{x_{t}}$, (3) $v_{t+1}  = v_{t}+\alpha_{t}\delta_{t}f_{x_{t}}$, (4) $\theta_{t+1}  =  \Gamma(\theta_{t}+\beta_{t}\delta_{t}\psi_{x_{t}a_{t}})$. In the above-mentioned equations, $\hat{J}_t$, $\delta_t$, $v_t$ and $\theta_t$ are the average reward, TD-error, critic and actor parameters at time $t$ respectively. The parameters $\epsilon_{t}, \alpha_{t}$ and $\beta_{t}$ are step-size parameters where $\alpha_{t} > \beta_{t}$ and $\epsilon_{t} = c\alpha_{t}$ for a positive scalar $c$. $\Gamma:\mathbb{R}^d \rightarrow \mathbb{R}^d$ is a projection operator ensuring that actor parameter updates remain within a compact set \cite{Bhatnagar2009}.
%
%Since $\hat{d}^\pi (x)$ is a stationary distribution, we have that the proof of convergence for Robust AC-PG holds in the regular AC-PG case \cite{Bhatnagar2009} as stated in Theorem \ref{thm:1}.
%
%\begin{theorem}
%\label{thm:1}
%Suppose $J(\pi)=\sum_{x\in X}\hat{d}^{\pi}(x)\sum_{a\in A}\pi(x,a)R(x,a)$ is the robust average performance objective, $\{\alpha_k\}_{k=0}^{\infty}, \{\beta_k\}_{k=0}^{\infty}, \{\eta_k=c\alpha_k\ \vert c>0\}_{k=0}^{\infty}$ are step size sequences where $\alpha_k > \beta_k$, and $\pi_{\theta}$ is an arbitrary policy parameterized by $\theta$. Then, by optimizing with respect to $J(\pi)$, RAC-PG converges to a local optimum policy parameterization $\theta^*$ following the results of \cite{Bhatnagar2009}.
%\end{theorem}
%
%The proof is in the supplementary material and mostly follows Bhatnagar's structure, but contains significant differences due to generalizing to Robust MDPs.

\section{Robust Options Policy Iteration (ROPI)}
\label{sec:rspi}

%Initially, a skill policy (for example, the ASAP policy) is provided to the algorithm with parameters $\theta\in \mathbb{R}^m$ and critic parameters $w \in \mathbb{R}^d$. In addition, a set of features $\phi\in \mathbb{R}^d$ are provided. Finally, a

Given the robust policy gradient, we now present Robust Options Policy Iteration (ROPI) defined as Algorithm \ref{alg:my_alg}. A parameterized uncertainty set $p_\mu$ with parameters $\mu$ and a nominal model without uncertainty $\hat{p}_\mu$ are provided as input to ROPI. In practice, the uncertainty set, for example, can be confidence intervals specifying plausible values for the mean of a normal distribution. The nominal model can be the same normal distribution without the confidence intervals. At each iteration, trajectories are generated (Line 3) using the nominal model $\hat{p}_\mu$ and the current policy $\pi_{\theta}$. These trajectories are utilized to learn the critic parameters $w$ in line $4$ using Robust Projected Value Iteration (RPVI) \cite{Tamar2014}.  As stated in the background section, RPVI converges to a fixed point. Once it has converged to this fixed point, we then use this critic to learn the option policy parameters $\theta$ (Line 5) using the R-PG update. This is the policy improvement step. This process is repeated until convergence. The convergence theorem is presented as Theorem \ref{thm:2}.   

%\begin{algorithm}[tb] 
%\caption{Robust Skills Policy Iteration} 
%\begin{algorithmic}[1] 
%%\Require ~\\ 
%%$w \in \mathbb{R}^d$ - The approximate value function parameters, 
%%$\phi \in \mathbb{R}^m$  - A set of features, $\pi_{\theta}$- An arbitrary parameterized skill policy with parameters $\theta$,  $\gamma$ - The discount factor, $M$ - The max. number of iterations for robust AC-PG, $p_\mu$ - An uncertainty set, $\hat{p}_\mu$ - A nominal model
%% 
%%\Repeat
%\STATE \textbf{Update critic:}
%\STATE $\tau \sim (\pi_{\theta}, \hat{p}_\mu)$ \COMMENT{Generate trajectories}
%\STATE Call RPVI($\tau$)
%%\Function {RPVI}{$\tau$}
%%\STATE $w_{t}=(\Phi^{T}\omega\Phi)^{-1}(\Phi^{T}\omega\mathbf{r}+\gamma\Phi^{T}\omega \sigma_{\pi_{\theta}}\{\Phi w_{t-1}\})$
%%\STATE \Return $w_{t}$
%%\EndFunction
%\STATE Set $\hat{w} = w_{t}$
%
%\STATE \textbf{Update actor:}
%\STATE Draw action $a_t$, observe $s_{t+1}, r_{t+1}$
%\STATE TD: $\delta_t = r_{t+1} + w_t^Tf_{s_{t+1}} - w_t^Tf_{s_{t}}$
%\STATE Actor: $\theta_{t+1} = \Gamma(\theta_t + \beta_t \delta_t \psi_{s_{t}a_{t}})$
%\STATE $\theta =  \theta_M$ \COMMENT{Update policy parameters}
%\STATE \textbf{Until max iterations or convergence}
%%\Until {Convergence}
%\STATE  {\bfseries return:}  {$\pi_{\theta}$} 
%\COMMENT{ The robust skills policy} 
%\end{algorithmic} 
%\label{alg:my_alg}
%\end{algorithm}

\begin{algorithm}[tb] 

\caption{Robust Options Policy Iteration (ROPI)} 

\begin{algorithmic}[1] 
\Require ~\\ 
$w \in \mathbb{R}^d$ - The approximate value function parameters, 
$\phi \in \mathbb{R}^m$  - A set of features, $\pi_{\theta}$- An arbitrary parameterized option policy with parameters $\theta$,  $\gamma$ - The discount factor, $p_\mu$ - An uncertainty set, $\hat{p}_\mu$ - A nominal model
 
\Repeat
%\State \textbf{Policy Evaluation:}
\State $\tau \sim (\pi_{\theta}, \hat{p}_\mu)$ \Comment{Generate trajectories}
\State \textbf{PE}: $w_{t} = (\Phi^{T}\omega\Phi)^{-1}(\Phi^{T}\omega\mathbf{r}+\gamma\Phi^{T}\omega \sigma_{\pi_{\theta}}\{\Phi w_{t-1}\})$ \Comment{Perform RPVI}
%\State \textbf{Policy Improvement:}
%\State Using $\pi_\theta$ and $\hat{p}_\mu$, draw action $a_t$, observe $s_{t+1}, r_{t+1}$
\State \textbf{PI}: $\theta_{t+1} =\theta_{t}+\alpha_{t}\nabla_{\theta} J_{\theta, w_{t}}(\pi_{\theta})$ \Comment{Update policy parameters}
\Until {Convergence}
\State  {\bfseries return:}  {$\pi_{\theta}$} 
\Comment{ The robust option policy} 

\end{algorithmic} 
\label{alg:my_alg}

\end{algorithm}

\begin{theorem}
Let $\pi$ and $f_{w}$ be any differentiable function approximators
for the option policy and value function respectively that satisfy the compatibility
condition derived above and for which the option policy is differentiable
up to the second derivative with respect to $\theta.$ That is, $\max_{\theta,x,a,i,j}\vert\frac{\partial^{2}\pi(x,a)}{\partial\theta_{i}\partial\theta_{j}}\vert<B<\infty.$
Define $\{\alpha_{k}\}_{k=0}^{\infty}$ be any step-size sequence
satisfying $\lim_{k\rightarrow\infty}\alpha_{k}=0$ and $\sum_{k}\alpha_{k}=\infty$.
Then the sequence $\{J(\pi_{k})\}_{k=0}^{\infty}$ defined by any
$\theta_{0}$, $\pi_{k}(\cdot,\cdot,\theta_{k})$ and 

\vspace{-0.4cm}
\begin{align*}
w_{k} & =w\enspace s.t.\enspace\sum_{x}\hat{d}^{\pi_{k}}(x)\sum_{a\in A}\frac{\partial\pi_{k}(x,a)}{\partial\theta} \biggl[Q^{\pi_{k}}(x,a)-f_{w}(x,a) \biggr]\frac{\partial f_{w}(x,a)}{\partial w}=0\\
\theta_{k+1} & =\theta_{k}+\alpha_{k}\sum_{x}\hat{d}^{\pi_{k}}(x)\sum_{a}\frac{\partial\pi_{k}(x,a)}{\partial\theta}f_{w_{k}}(x,a)\enspace,
\end{align*}

converges such that $\lim_{k\rightarrow\infty}\frac{\partial J(\pi_{k})}{\partial\theta}=0$.
\label{thm:2}
\end{theorem}


